AllSight: A Low-Cost and High-Resolution Round Tactile Sensor with Zero-Shot Learning Capability

Tactile sensing is a necessary capability for a robotic hand to perform fine manipulations and interact with the environment. Optical sensors are a promising solution for high-resolution contact estimation. Nevertheless, they are usually not easy to fabricate and require individual calibration in order to acquire sufficient accuracy. In this letter, we propose AllSight, an optical tactile sensor with a round 3D structure potentially designed for robotic in-hand manipulation tasks. AllSight is mostly 3D printed making it low-cost, modular, durable and in the size of a human thumb while with a large contact surface. We show the ability of AllSight to learn and estimate a full contact state, i.e., contact position, forces and torsion. With that, an experimental benchmark between various configurations of illumination and contact elastomers are provided. Furthermore, the robust design of AllSight provides it with a unique zero-shot capability such that a practitioner can fabricate the open-source design and have a ready-to-use state estimation model. A set of experiments demonstrates the accurate state estimation performance of AllSight.

==> design_eval.tex <==
Creating a 3D surface tactile sensor is a challenging task due to its sensitivity to numerous parameters, which hinder its ability to adapt to different robotic applications. Developing a deformable gel and rigid shell presents several challenges and may result in imaging artifacts, in particular for the marked elastomer. Pouring clear gel requires careful consideration to avoid bubbles, while applying adhesive between layer needs to be uniform to remove excess air. A trade-off exists between layer thickness and resolution, with thinner layers offering higher resolution but being more susceptible to damage. Similarly, the coating thickness also affects performance. We conducted multiple iterations during the design process, experimenting with various thicknesses, adhesion and coating types, and part fabrication to create a robust design that enhances adaptation, reliability, and amenable to large-scale production without compromising sensing performance. Our gel is clearer and requires fewer fabrication steps compared to previous sensor designs. 


% \subsubsection{illumination effects }
% maybe ill only add 1 picture that present everything, how dont think we have the ability to give the right metrics
% \begin{enumerate}
%     \item different coating ( aluminum flake, silicone ink, silicone ink + gel
%     \item different rigid shells ( epoxy, crystal clear SLA, with/out polish)
%     \item different gel width (3-7 mm)
%     \item with and without light-piping / structured light
% \end{enumerate}



\subsubsection{Durability }
To start with, we tested the mechanical characteristics of Allsight to determine its resistance to wear and tear. We performed a randomized probing process over the entire surface of Allsight X times. After each round, we inspected the gel for any tears or imaging defects by measuring the SSIM between the starting image and observing its light transmittance.


==> original_table.tex <==
This is the table in the initial submission to RA-L.

%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\caption{\small State-of-the-art comparison of optical-based tactile sensors}
\label{tb:sota}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lc ccc cc cccc ccc}
\hline
\multirow{2}{*}{Sensor} && \multicolumn{3}{c}{Transduction Method}   & Surface  & Open-  & \multicolumn{4}{c}{Contact state$^*$} & Max. & Dimension & Weight   \\ \cline{3-5}\cline{8-11}
 && Camera & PS & Markers & shape & source & $\ve{x}$ & $f_z$ & $f_x,f_y$ & $\tau$ & $f_z$ (N) & (mm) & (g) \\ % & ($mm^2$)
\hline

GelSight (2017) & \cite{yuan2017gelsight} & \checkmark & \checkmark &  & 2D & & & \checkmark & \checkmark & \checkmark & 25 & $40\times80\times40$ & -\\ %252 (18X14) 

\rowcolor{Gray}
TacTip (2018) & \cite{ward2018tactip} & \checkmark & & \checkmark & 3D & \checkmark    & \checkmark &&& & - & $40\times40\times85$ & - \\ %2,500 

Romero et al. (2020) & \cite{romero2020soft} & \checkmark & \checkmark &  & Half 3D & & &&& & - & $28\times30\times35$ & - \\ % (half) 2,069 

\rowcolor{Gray}
GelTip (2020) & \cite{gomes2020geltip} & \checkmark & \checkmark &  & 3D & & \checkmark &&& & - & $30\times30\times100$ & -\\ %2,513 

% Lin et al. \cite{lin2020curvature} & \checkmark & & & \checkmark & & Deformation & - & 2,510 & $\varnothing40$  \\

Omnitact (2020) & \cite{padmanabha2020omnitact} & $5\times$\checkmark & \checkmark & & 3D & & \checkmark &&& & - & $30\times30\times33$ & - \\% 3,110 (30 dia.)

\rowcolor{Gray}
DIGIT (2020) & \cite{lambeta2020digit} & \checkmark & \checkmark & \checkmark & 2D & & &&& & - & $20\times27\times18$ & 20 \\ % 304 (25X19) 

GelStereo (2021) & \cite{cui2021self} & $2\times$\checkmark & \checkmark & & 2D & & &&& & - & - & -\\

\rowcolor{Gray}
GelSight wedge (2021) & \cite{wang2021gelsight} & \checkmark & \checkmark & \checkmark & 2D & & & & &  & - & - & - \\ % Force map is not given explicitly 768 (32X24) 

Insight (2022) & \cite{sun2022soft} & \checkmark & \checkmark &  & 3D  & & \checkmark & \checkmark & \checkmark & & 2   & $40\times40\times 70$ & - \\ % 4,800  

\rowcolor{Gray}
GelSlim 3.0 (2022) & \cite{taylor2022gelslim} & \checkmark & \checkmark & \checkmark & 2D & \checkmark & & \checkmark & \checkmark & & - & $20\times37\times80$ & 45 \\ % 1,200 (30x40) 

DenseTact (2023) & \cite{do2023densetact}  & \checkmark & \checkmark &  & 3D & &  & \checkmark & \checkmark & \checkmark & [-11, 3] & $30\times30\times43$ & - \\ % I do not treat the noise as markers 1,560 (31.5dia) 
\hline
\rowcolor{Gray}
\se & Ours & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 15 & $26\times28\times38$ & 15 \\ \hline

\multicolumn{14}{l}{\footnotesize $^*$$\ve{x}$ denotes contact position; $f_z$ denotes normal force; $f_x$ and $f_y$ denote tangential forces; and $\tau$ denotes torsion about the normal at the contact surface.}\\
% \multicolumn{14}{l}{\footnotesize "-" denotes that the information is not specified.}
\end{tabular}
\end{adjustbox}
\vspace{-0.5cm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%
